Network regression and supervised centrality estimation

The centrality in a network is often used to measure nodes' importance and model network effects on a certain outcome. Empirical studies widely adopt a two-stage procedure, which first estimates the centrality from the observed noisy network and then infers the network effect from the estimated centrality, even though it lacks theoretical understanding. We propose a unified modeling framework to study the properties of centrality estimation and inference and the subsequent network regression analysis with noisy network observations. Furthermore, we propose a supervised centrality estimation methodology, which aims to simultaneously estimate both centrality and network effect. We showcase the advantages of our method compared with the two-stage method both theoretically and numerically via extensive simulations and a case study in predicting currency risk premiums from the global trade network.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> output/trade_premium/trade_premium_epsy_1999_gap_gdp_miter1000.tex <==
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{tab:rx-sigma} 
\begin{tabular}[t]{lrrr}
\toprule
Method & $\widehat\sigmay$ & $\widehat\sigmaa$ & $\hd$ \\
\midrule
Two-stage-naive & 0.0018554 & 0.0019839& 0.0020164\\
Two-stage & 0.0018107 & 0.0019839 & 0.0020164\\
$\supercentcv$ & 0.0000002 & 0.0024671 & 0.0013041\\
\bottomrule
\end{tabular}
\end{table}

==> output/trade_premium_old/10_year_return_gap3.tex <==
\begin{table}

\caption{\label{tab:tbl:excess-return-3}The 10-year average return}
\centering
\begin{tabular}[t]{lllllll}
\toprule
\multicolumn{1}{c}{} & \multicolumn{2}{c}{Top/Bottom 3} & \multicolumn{2}{c}{Top/Bottom 4} & \multicolumn{2}{c}{Top/Bottom 5} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7}
 & Hub & Authority & Hub & Authority & Hub & Authority\\
\midrule
SuperCENT CV & 0.0025 & 0.0046 & 0.003 & 0.0036 & 0.003 & 0.0036\\
Two-stage & 0.0025 & 0.0004 & 0.0028 & 0.0004 & 0.0028 & -0.0001\\
Relative difference & 0.4\% & 943.4\% & 5.6\% & 691.1\% & 7.9\% & 4 205.2\%\\
\bottomrule
\end{tabular}
\end{table}


==> output/trade_premium_old/10_year_return_gap5.tex <==
\begin{table}
\caption{\label{tab:tbl:excess-return}The 10-year average return}
\vspace{-1em}
\centering
\renewcommand*{\arraystretch}{1}
\begin{tabular}[t]{lllllll}
\toprule
\multicolumn{1}{c}{} & \multicolumn{2}{c}{Top/Bottom 3} & \multicolumn{2}{c}{Top/Bottom 4} & \multicolumn{2}{c}{Top/Bottom 5} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7}
 & Hub & Authority & Hub & Authority & Hub & Authority\\
\midrule
% SuperCENT CV
{$\supercent$} & 0.0031 & 0.0021 & 0.0036 & 0.0019 & 0.0033 & 0.0014\\
Two-stage & 0.0003 & -0.0014 & 0.0008 & -0.001 & 0.001 & -0.0006\\
Relative difference & 1 136\% & 253\% & 338\% & 285\% & 237\% & 320\%\\
\bottomrule
\end{tabular}
% \vspace{-1em}
\end{table}


==> output/trade_premium_old/trade_premium_1999_gap10_gdp_miter1000.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Mon, Sep 06, 2021 - 00:41:07
\begin{table} \centering 
  \caption{The summary table of the regression comparing three methods in terms of coefficient estimation, standard error (in parenthesis) and the significant level (by asterisks). 
%   \dyR{we do not need the rows 1, 2, 4, do we?}
%\dyR{why is $0.0081<0.0083$. two stage should be wider than two-stage adhoc, right?}
%\jcB{You are right. When calculating $Cov(\betax)$, $\sigma_y^2$ was estimated with $SSE/(n-p-1)$, but should be $SSE/(n-p)$ because the intercept is already included in the design matrix.}
%\dyR{are you saying that for two-stage-adhoc and two-stage, you used different estimates of $\sigma_y^2$? if you use the same, it does not matter whether $n-p$ or $n-p-1$ was used. two-stage should always be wider than two-stage-adhoc. moreover, we have been using $n-p-2$ throughout the narrative of the paper. what did you use exactly?}
  } 
  \label{tab:rx-summary} 
  % \renewcommand*{\arraystretch}{.9}
\begin{tabular}{@{\extracolsep{5pt}}lllllll} 
\hline 
% & \multicolumn{3}{c}{\textit{Dependent variable:} Risk premium} \\ \\
% \cline{2-4} 
% \\[-1.8ex] & \multicolumn{3}{c}{Risk premium} \\ 
 & \multicolumn{2}{c}{Two-stage-adhoc} & \multicolumn{2}{c}{Two-stage} & \multicolumn{2}{c}{$\supercentcv$} \\ 
\hline 
 GDP share {$\betax$} & $-$0.0159$^{*}$ & (0.0083) & $-$0.0159$^{*}$ & (0.0083) & $-$0.0162$^{***}$ & (0.0037)\\ 
 Hub {$\betau$} & $-$0.0011 & (0.0006)& $-$0.0011$^{*}$& (0.0006) &  $-$0.0021$^{***}$ &  (0.0002)\\ 
 Authority {$\betav$}& $-$0.0005& (0.0006) & $-$0.0005& (0.0006) & $-$0.0003 &  (0.0003) 
    \\ \hline
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} 
\end{tabular} 
\vspace{-1em}
\end{table} 


==> output/trade_premium_old/trade_premium_epsy_1999_gap_gdp_miter1000.tex <==
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{tab:rx-sigma} 
\begin{tabular}[t]{lrrr}
\toprule
Method & $\widehat\sigmay$ & $\widehat\sigmaa$ & $\hd$ \\
\midrule
Two-stage-naive & 0.0018554 & 0.0019839& 0.0020164\\
Two-stage & 0.0018107 & 0.0019839 & 0.0020164\\
$\supercentcv$ & 0.0000002 & 0.0024671 & 0.0013041\\
\bottomrule
\end{tabular}
\end{table}
